Incremental Methods for Weakly Convex Optimization

Incremental methods are widely utilized for solving finite-sum optimization problems in machine learning and signal processing. In this paper, we study a family of incremental methods -- including incremental subgradient, incremental proximal point, and incremental prox-linear methods -- for solving weakly convex optimization problems. Such a problem class covers many nonsmooth nonconvex instances that arise in engineering fields. We show that the three said incremental methods have an iteration complexity of $O(\varepsilon^{-4})$ for driving a natural stationarity measure to below $\varepsilon$. Moreover, we show that if the weakly convex function satisfies a sharpness condition, then all three incremental methods, when properly initialized and equipped with geometrically diminishing stepsizes, can achieve a local linear rate of convergence. Our work is the first to extend the convergence rate analysis of incremental methods from the nonsmooth convex regime to the weakly convex regime. Lastly, we conduct numerical experiments on the robust matrix sensing problem to illustrate the convergence performance of the three incremental methods.

==> untitled folder/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Incremental Methods for Weakly Convex Optimization}{X. Li, Z. Zhu, A. M.-C. So, J. D. Lee}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{ Incremental Methods for \\ Weakly Convex Optimization
%	\thanks{ 
%		\funding{X. Li was partially supported by the University Development Fund UDF01001808 of CUHK (SZ).  Z. Zhu was partially supported by NSF Grant CCF-2008460. A. M.-C. So was partially supported by the Hong Kong Research Grants Council (RGC) General Research Fund (GRF) Project CUHK 14208117 and the CUHK Research Sustainability of Major RGC Funding Schemes Project 3133236.}
%}
}

% Authors: full names plus addresses.
\author{Xiao Li\thanks{School of Data Science, The Chinese University of Hong Kong, Shenzhen. 
		(\email{lixiao@cuhk.edu.cn}, \url{ https://sites.google.com/view/xli}).}
\and Zhihui Zhu\thanks{Department of Electrical and Computer Engineering, University of Denver. (\email{zhihui.zhu@du.edu}, \url{http://mysite.du.edu/\~zzhu61/}).}
\and Anthony Man-Cho So\thanks{Department of Systems Engineering and Engineering Management, The Chinese University of Hong Kong. 
	(\email{manchoso@se.cuhk.edu.hk}, \url{http://www.se.cuhk.edu.hk/\~manchoso}). }
\and Jason D Lee\thanks{ Department of  Electrical Engineering,   Princeton University. (\email{jasonlee@princeton.edu}, \url{https://jasondlee88.github.io/}).
}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> untitled folder/macro.tex <==
\usepackage{array}
\usepackage{url}
%\usepackage[hidelinks]{hyperref}
\usepackage{amsmath,amssymb,amsbsy}
\usepackage{paralist}
\usepackage{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{comment}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{bm}
\usepackage{framed}
\usepackage{fancyhdr}
\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}

% Theorems
%\def \remarks {\noindent {\bf Remarks.}\ \ }
\newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
\newtheorem{lem}{Lemma}%[section] %%    with section number.
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
%\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{prob}{Problem}
\newtheorem{obs}{Observation}
\newtheorem{assum}{Assumption}
\newtheorem*{goal}{Plan}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma} 
\newtheorem{update}{Updating rule}
\newtheorem{fact}{Fact}%[section]
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}


% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
\newcommand{\btab}{\begin{tabular}}
\newcommand{\etab}{\end{tabular}}

% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

% probability and stat
\renewcommand{\P}[1]{\Pr\left[#1\right]}
\newcommand{\E}{\operatorname{E}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}

\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\starT}{{\star\mathrm{T}}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\Sign}{\operatorname{Sign}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\supp}{\operatorname{supp}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{argmin}}
\DeclareMathOperator*{\argmax}{\text{argmax}}
\newcommand{\prox}{\operatorname{prox}}
\newcommand{\dom}{\operatorname{dom}}
\def \st {\operatorname*{subject\ to\ }}
% other
\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}
\newcommand{\purple}[1]{{\color{purple}{#1}}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}





\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vdelta}{\vct{\delta}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{{\bm I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bm 0}}
\newcommand{\mone}{{\bf 1}}
\newcommand{\mPi}{{\bf \Pi}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note: } #1]}}
\newcommand{\notezz}[1]{\textcolor{blue}{\bf [{\em Note: zz:} #1]}}
\newcommand{\notexli}[1]{\textcolor{blue}{\bf [{\em Note: xli:} #1]}}
\newcommand{\revise}[1]{\textcolor{red}{#1}}
\newcommand{\edit}[1]{\textcolor{blue}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\newcommand{\Poff}{\mathcal{P}_{\textup{off}}}
\newcommand{\Pon}{\mathcal{P}_{\textup{diag}}}



\usepackage[framemethod=tikz]{mdframed}
\newcommand{\block}[1]{
	\begin{mdframed}[
		nobreak=true,
		leftmargin =0pt,
		rightmargin =0pt,
		innerleftmargin =5pt,
		innerrightmargin =5pt,
		%skipabove=8pt,
		innertopmargin=4pt,
		backgroundcolor=black!10,
		rightline=false,leftline=false]{#1}
\end{mdframed}}

\newcommand{\blk}[2][]{
	\begin{mdframed}[
		frametitle={#1},
		frametitlefont={\sffamily\bfseries},
		nobreak=true,
		leftmargin =0pt,
		rightmargin =0pt,
		innerleftmargin =4pt,
		innerrightmargin =4pt,
		skipabove=4pt,
		innertopmargin=4pt,
		%backgroundcolor=black!10,
		topline=true, bottomline=true,
		rightline=true,leftline=true]{#2}
\end{mdframed}}
